Integrating Distributed Energy Resources: Optimal Prosumer Decisions and Impacts of Net Metering Tariffs

The rapid growth of the behind-the-meter (BTM) distributed generation has led to initiatives to reform the net energy metering (NEM) policies to address pressing concerns of rising electricity bills, fairness of cost allocation, and the long-term growth of distributed energy resources. This article presents an analytical framework for the optimal prosumer consumption decision using an inclusive NEM X tariff model that covers existing and proposed NEM tariff designs. The structure of the optimal consumption policy lends itself to near closed-form optimal solutions suitable for practical energy management systems that are responsive to stochastic BTM generation and dynamic pricing. The short and long-run performance of NEM and feed-in tariffs (FiT) are considered under a sequential rate-setting decision process. Also presented are numerical results that characterize social welfare distributions, cross-subsidies, and long-run solar adoption performance for selected NEM and FiT policy designs.

==> AdoptionDyn.tex <==
To capture the adoption dynamics under each metering policy, we use the developed nonlinear feedback model for the DER adoption
processes in \cite{Tong_DERdynamics:20TAC}, which also governs the rate-setting process in section \ref{sec:RegulatorProblem} (Fig.\ref{fig:Dynamics}). The system state $\sigma_n = (\pi_n, \gamma_n)$ consists of the tariff at the beginning of a pricing cycle $\pi_n$ determined based on (\ref{eq:Ramseymaximization}), and the fraction of adopters at the end of the pricing cycle $\gamma_n$. The system state evolution has the form
\begin{equation}\label{eq:SystemState}
    \sigma_{n+1}=f_{n}\left(\sigma_{n}, \chi_{n}\right), \quad\left\{\begin{array}{l}
\sigma_{n}=\left(\pi_{n}, \gamma_{n}\right) \\
\chi_{n}=\left(\theta_{n}, \xi_{n}\right)
\end{array}\right.,
\end{equation}
where the exogenous process $\chi_{n}=(\theta_n,\xi_n)$ consists of the expected utility fixed cost $\theta_n$, and the per-unit DER installation cost $\xi_n$. The specific form of the closed-loop system $f_n$ depends on the tariff design given in (\ref{eq:NextPeriodTariff}) and the technology adoption model.
\begin{figure}[htbp]
    \centering
    \includegraphics[scale=0.45]{Dynamics.eps}
    \caption{Nonlinear feedback model of DER adoption.}
    \label{fig:Dynamics}
\end{figure}

\subsection{Technology adoption model}\label{subsec:AdoptionModel}
The DER adoption model $h_n$ is assumed to be primarily based on the DER investment payback time. As in \cite{Tong_DERdynamics:20TAC}, the widely used $S$-curve was utilized to model the adoption process of the customers \cite{bassModel:1969MS}. The \textit{DER adoption curve} $s(t;\pi,\xi)$ parametrized by time $t$ is
\begin{equation}\label{eq:AdoptionCurve}
    s(t;\pi,\xi) = \gamma_\infty(\pi,\xi) \eta(t),
\end{equation}
where $\gamma_\infty(\pi,\xi)$ is the DER \textit{market potential}, and $\eta(t)$ is the \textit{cumulative installed fraction}, which can take the form of Bass diffusion model \cite{bassModel:1969MS} satisfying $\eta(0)=0$ and $\lim_{t \rightarrow \infty} \eta(t)=1$. 
\par The adoption curve given by (\ref{eq:AdoptionCurve}) does only describe the evolution of the adoption when the tariff $\pi$ and the exogenous DER cost $\xi$ are fixed, before reaching $\gamma_\infty(\pi,\xi)$.  To capture the diffusion dynamics, the dynamical equation in \cite{Tong_DERdynamics:20TAC} is used as follows
\begin{equation}\label{eq:dynamicallEquationforGamma}
    h_{n}: \gamma_{n+1}= \begin{cases}\gamma_{n},  \hspace{2.3cm} \text { if } \gamma_{\infty}\left(\pi_{n+1}, \xi_{n+1}\right)<\gamma_{n} ; \\ s\left(1+\eta^{-1}\left(\frac{\gamma_{n}}{\gamma_{\infty}\left(\pi_{n+1},\xi_{n+1}\right)}\right) ; \pi_{n+1}, \xi_{n+1}\right),  \text {o.w., }\end{cases}
\end{equation}
which together with (\ref{eq:NextPeriodTariff}) specifies the nonlinear model in (\ref{eq:SystemState}).
\subsection{Performance metrics}\label{subsec:PerformanceMetrics}
Three performance metrics are used to thoroughly analyze the long-run performance and effect of a tariff on: a) social welfare, b) cross-subsidy, and c) BTM DER adoption.
\subsubsection{Social welfare}
We adopt a generalized notion of the expected social welfare $W^\pi_\gamma$, where the customers' surplus, utility's surplus, and environmental benefits externality brought by the diffusion of BTM DER are all considered.
\begin{equation}\label{eq:welfare}
W^{\pi}_{\gamma_n}= \sum_{j=1}^J \mathbb{E} \bigg( S_{cu}^\pi (\bm{d}^*(r_j),\gamma_n) + S^\pi_{ut} (\bm{d}^*(r_j),\gamma_n) + \gamma_n \mathcal{E}(r_j)\bigg),
\end{equation}
where $\mathcal{E}(r_j) = \pi^e \mathbb{E}(r_j)$ is a linear function of the total BTM generation $r_j$.

\subsubsection{Cross-subsidy}
To evaluate cross-subsidies, the expected cost-shifts $\psi^\pi_{\gamma_n}$ from adopters to non-adopters is measured. Cost-shifts occur when the bill savings of the adopters $\Delta P_\pi\left(r_j\right)$ exceeds the utility's avoided cost due to BTM DER generation \cite{EdisonReport_Borlick_Wood}
\begin{equation}
    \label{eq:ProfitDefficit}
    \psi^\pi_{\gamma_n} = \sum_j \gamma  \mathbb{E}\left(\Delta P_\pi\left(r_j\right)- \pi^{\mbox{\tiny SMC}} r_j \right),
\end{equation}
where $\pi^{\mbox{\tiny SMC}}$ is the social marginal cost price of electricity \cite{Next10Report}, and $\Delta P^\pi\left(r_j\right)$ is the bill savings due to onsite DER given by
\begin{equation}
    \Delta P_\pi (r_j):= P_\pi({\bf 1}^{\top}\bm{d}^*_0) - P_\pi({\bf 1}^{\top}\bm{d}^*_p(r_j) - r_j),
\end{equation}
which is the difference between the payment under optimal consumption before and after installing the DER.
\subsubsection{Payback time and market potential}
To evaluate (\ref{eq:AdoptionCurve}), we consider the following parametric form of the market potential function \cite{beckMktPotential:2009}
\begin{equation}\label{eq:MktPoten}
    \gamma_\infty(\pi,\xi) = \gamma^{\mbox{\tiny MS}} e^{\varepsilon t_{pb}^\pi},
\end{equation}
where $\varepsilon$ is the payback sensitivity, and the payback time is the solution of
\begin{equation}
\label{eq:TNPpaybackTime}
    t_{pb}^\pi(r,\xi) =\min_{t^\ast}\left\{t^\ast: \sum_{t=0}^{t^\ast} \left(\frac{1-\nu}{1+\zeta}\right)^t  \mathbb{E}\left(\Delta P_{\pi,t}(r_t)\right) \geq \xi \right\},
\end{equation}
where $\nu,\zeta \in [0,1)$ are the BTM DER system degradation factor and interest rate, respectively, $t$ is the compounding rate.
